A new derivation of the Hubble constant from $\gamma$-ray attenuation using improved optical depths for the Fermi and CTA era

We present $\gamma$-ray optical-depth calculations from a recently published extragalactic background light (EBL) model built from multiwavelength galaxy data from the Hubble Space Telescope Cosmic Assembly Near-Infrared Deep Extragalactic Legacy Survey (HST/CANDELS). CANDELS gathers one of the deepest and most complete observations of stellar and dust emissions in galaxies. This model resulted in a robust derivation of the evolving EBL spectral energy distribution up to $z\sim 6$, including the far-infrared peak. Therefore, the optical depths derived from this model will be useful for determining the attenuation of $\gamma$-ray photons coming from high-redshift sources, such as those detected by the Large Area Telescope on board the Fermi Gamma-ray Space Telescope, and for multi-TeV photons that will be detected from nearby sources by the future Cherenkov Telescope Array. From these newly calculated optical depths, we derive the cosmic $\gamma$-ray horizon and also measure the expansion rate and matter content of the Universe including an assessment of the impact of the EBL uncertainties. We find $H_{0}=61.9$ $^{+2.9}_{-2.4}$ km s$^{-1}$ Mpc$^{-1}$ when fixing $\Omega_{m}=0.32$, and $H_{0}=65.6$ $^{+5.6}_{-5.0}$ km s$^{-1}$ Mpc$^{-1}$ and $\Omega_{m}=0.19\pm 0.07$, when exploring these two parameters simultaneously.

==> table.tex <==
\begin{table}
	\centering
	\caption{This is an example table. Captions appear above each table.
	Remember to define the quantities, symbols and units used.}
	\label{tab:example_table}
	\begin{tabular}{lccr} % four columns, alignment for each
		\hline
		A & B & C & D\\
		\hline
		1 & 2 & 3 & 4\\
		2 & 4 & 6 & 8\\
		3 & 5 & 7 & 9\\
		\hline
	\end{tabular}
\end{table}
